PlantTracing: Tracing Arabidopsis Thaliana Apex with CenterTrack

This work applies an encoder-decoder-based machine learning network to detect and track the motion and growth of the flowering stem apex of Arabidopsis Thaliana. Based on the CenterTrack, a machine learning back-end network, we trained a model based on ten time-lapsed labeled videos and tested against three videos.

==> ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{1}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Plant-Tracer}
A.~M. Guercio, Y.~Mao, V.~N. Carvalho, J.~Zhang, C.~Li, Z.~Ren, W.~Zhao,
  Y.~Wang, and E.~D. Brenner, ``Plant tracer: A program to track and quantify
  plant movement from cellphone captured time-lapse movies.'' \emph{Bioscene:
  Journal of College Biology Teaching}, vol.~45, no.~3, pp. 14--21, 2019.

\bibitem{block-matching}
J.~Lu and M.~L. Liou, ``A simple and efficient search algorithm for
  block-matching motion estimation,'' \emph{IEEE Transactions on Circuits and
  Systems for Video Technology}, vol.~7, no.~2, pp. 429--433, 1997.

\bibitem{CenterTrack}
X.~Zhou, V.~Koltun, and P.~Krähenbühl, ``Tracking objects as points,'' 2020.

\bibitem{CenterNet}
X.~Zhou, D.~Wang, and P.~Krähenbühl, ``Objects as points,'' 2019.

\bibitem{encoderdecoder}
K.~Cho, B.~van Merrienboer, C.~Gulcehre, D.~Bahdanau, F.~Bougares, H.~Schwenk,
  and Y.~Bengio, ``Learning phrase representations using rnn encoder-decoder
  for statistical machine translation,'' 2014.

\bibitem{deformableCNN}
J.~Dai, H.~Qi, Y.~Xiong, Y.~Li, G.~Zhang, H.~Hu, and Y.~Wei, ``Deformable
  convolutional networks,'' 2017.

\bibitem{DLA}
F.~Yu, D.~Wang, E.~Shelhamer, and T.~Darrell, ``Deep layer aggregation,'' 2019.

\bibitem{kingma2017adam}
D.~P. Kingma and J.~Ba, ``Adam: A method for stochastic optimization,'' 2017.

\end{thebibliography}

